AutoCoder: Enhancing Code Large Language Model with \textsc{AIEV-Instruct}

We introduce AutoCoder, the first Large Language Model to surpass GPT-4 Turbo (April 2024) and GPT-4o in pass@1 on the Human Eval benchmark test ($\mathbf{90.9\%}$ vs. $\mathbf{90.2\%}$). In addition, AutoCoder offers a more versatile code interpreter compared to GPT-4 Turbo and GPT-4o. It's code interpreter can install external packages instead of limiting to built-in packages. AutoCoder's training data is a multi-turn dialogue dataset created by a system combining agent interaction and external code execution verification, a method we term \textbf{\textsc{AIEV-Instruct}} (Instruction Tuning with Agent-Interaction and Execution-Verified). Compared to previous large-scale code dataset generation methods, \textsc{AIEV-Instruct} reduces dependence on proprietary large models and provides execution-validated code dataset. The code and the demo video is available in \url{https://github.com/bin123apple/AutoCoder}.

==> Sections/6_Limitation_Discussion.tex <==
\section{Limitation and Discussion}



==> Sections/old_2_Related_Work.tex <==
\section{Related Work}
\begin{enumerate}
    \item besides what we have listed right now. Do you need to discuss reasoning problems? they may have some common features which are motivation of our design
    \begin{enumerate}
        \item complex: search space is big -\> we start from the target
        \item one path can benefit from the intermediate results from other paths: ToT cannot do that or has to introduce extra complexity. 
        \item solutions are restricted by the conditions -\> we introduce condition node
    \end{enumerate}
    \item GoT
\end{enumerate}

\textit{I-O} Prompting:
The most prevalent prompting method is Input-Output prompting. In this approach, one provides the conditions to the large model, which then produces answers following a token-level, left-to-right decision-making process \cite{zhang2022automatic}. This method is the default mode utilized by GPT-4.

\textit{CoT} Prompting \cite{wei2022chain}:
CoT prompting aims to guide the model in generating coherent text by establishing logical continuity. It is based on the assumption that by progressively expanding and supplementing chains of viewpoints and arguments, the model can generate more coherent and reasoning-based outputs. This method encourages the model to follow a sequential line of thought while answering questions, ensuring that the generated text is logically connected and coherent.

\textit{SC-CoT} Prompting \cite{wang2022self}:
SC-CoT prompting is an extension of the Chain-of-Thought method. It requires the model to maintain self-consistency and logical coherence while generating text. In other words, the generated content should be internally consistent and semantically connected. This consistency and logical flow can be ensured by leveraging large models to vote or score, followed by a selection process. By emphasizing the self-consistency of the model's output, this prompting method reduces logical errors and inconsistencies, thereby improving the quality of the generated text.

\textit{ToT} Prompting \cite{yao2023tree}:
ToT prompting employs structured prompts to assist the model in generating hierarchical and structured text. This method utilizes a tree-like structure to represent the relationships between different concepts, which serves as input prompts. The model can organize and reason about the text based on the structure of the tree, resulting in more accurate and structured answers. Tree of Thought also employs a voting or scoring mechanism to filter the generated results, thereby not only reducing errors but also decreasing computational costs. Tree-of-Thought prompting aims to provide richer semantic representation and improved logical organization, enhancing the model's reasoning capabilities and generation quality.

\textcolor{red}{Add current GoT Method, 1. Graph of thoughts: Solving elaborate problems with large language models. (Theory) 2. Mindmap: Knowledge graph prompting sparks graph of thoughts in large language models. 3. Beyond Chain-of-Thought, Effective Graph-of-Thought Reasoning in Large Language Models}

These are the four prompting methods, each offering guidance and constraints at different levels to facilitate language models in generating accurate, coherent, and reasoning-based text.
